Crossing exponent in the Brownian loop soup

We study the clusters of loops in a Brownian loop soup in some bounded two-dimensional domain with subcritical intensity $\theta \in (0,1/2]$. We obtain an exact expression for the asymptotic probability of the existence of a cluster crossing a given annulus of radii $r$ and $r^s$ as $r \to 0$ ($s >1$ fixed). Relying on this result, we then show that the probability for a macroscopic cluster to hit a given disc of radius $r$ decays like $|\log r|^{-1+\theta+ o(1)}$ as $r \to 0$. Finally, we characterise the polar sets of clusters, i.e. sets that are not hit by the closure of any cluster, in terms of $\log^\alpha$-capacity. This paper reveals a connection between the 1D and 2D Brownian loop soups. This connection in turn implies the existence of a second critical intensity $\theta = 1$ that describes a phase transition in the percolative behaviour of large loops on a logarithmic scale targeting an interior point of the domain.

==> subfiles/new.tex <==
\begin{lemma}
Let $H_\delta : (s,t) \in I_\leq^* \mapsto \Prob{ e^{-1} \overset{\Lc_\D^\theta}{\longleftrightarrow} \delta^t \Big\vert e^{-1} \overset{\Lc_\D^\theta}{\longleftrightarrow} \delta^s }$.
$H_\delta$ converges uniformly on each compact subspace of $I_\leq^*$ to $(s,t) \mapsto (t/s)^{-1+\theta}$.
\end{lemma}

\begin{proof}
As in the proof of Lemma \ref{L:crossing_tightness}, we can show that $(H_\delta)_{\delta >0}$ is tight, in the sense that for each decreasing sequence $(\delta_n)_{n \geq 0}$ converging to zero, we can extract a subsequence $(\delta_{n_k})_{k \geq 0}$ such that $(H_{\delta_{n_k}})_{k \geq 0}$ converges on each compact subspace of $I_\leq^*$ to a continuous function $H$.
For all $0 < s \leq t \leq u$ and $\delta>0$, we notice that
\[
H_\delta(s,	u) = H_\delta(s,t) H_\delta(t,u).
\]


If we knew the convergence of $H_\delta$, this equation would lead to
\[
H(1, u/s) = H(1, t/s) H(1, u/t),
\]
implying that $H(1,t) = t^{-a}$ for some exponent $a$. It is then easy to see that $a = 1-\theta$.
\end{proof}

Let $\delta > 0$ be small and $0 < s < t$. 
We start by noticing that
\begin{align*}
\Prob{e^{-1} \overset{\Lc_\D^\theta}{\longleftrightarrow} \delta^s}
= \Prob{e^{-1} \overset{\Lc_{\D \setminus \delta^t \D}^\theta}{\longleftrightarrow} \delta^s } + \Prob{e^{-1} \overset{\Lc_\D^\theta}{\longleftrightarrow} \delta^s , \text{not}~ e^{-1} \overset{\Lc_{\D \setminus \delta^t \D}^\theta}{\longleftrightarrow} \delta^s }.
\end{align*}
On the event that there is no crossing of $e^{-1} \D \setminus \delta^s \D$ by a cluster of loops in $\Lc_{\D \setminus \delta^{-t} \D}^\theta$, there is a crossing of $e^{-1} \D \setminus \delta^s \D$ by a cluster of $\Lc_\D^\theta$ if and only if there is a crossing $e^{-1} \D \setminus \delta^t \D$. The second right hand side term is therefore equal to
\begin{align*}
\Prob{e^{-1} \overset{\Lc_\D^\theta}{\longleftrightarrow} \delta^t , \text{not}~ e^{-1} \overset{\Lc_{\D \setminus \delta^t \D}^\theta}{\longleftrightarrow} \delta^s }
= \Prob{e^{-1} \overset{\Lc_\D^\theta}{\longleftrightarrow} \delta^t }
-  \Prob{e^{-1} \overset{\Lc_\D^\theta}{\longleftrightarrow} \delta^t , e^{-1} \overset{\Lc_{\D \setminus \delta^t \D}^\theta}{\longleftrightarrow} \delta^s  }.
\end{align*}
Now,
\begin{align*}
\Prob{e^{-1} \overset{\Lc_\D^\theta}{\longleftrightarrow} \delta^t , e^{-1} \overset{\Lc_{\D \setminus \delta^t \D}^\theta}{\longleftrightarrow} \delta^s  }
= \Prob{ \exists \wp \in \Lc_\D: \delta^s \overset{\wp}{\longleftrightarrow} \delta^t } \Prob{ e^{-1} \overset{\Lc_{\D \setminus \delta^t \D}^\theta}{\longleftrightarrow} \delta^s  } \\
+ \int_s^t \frac{\d}{\d u} \Prob{ \exists \wp \in \Lc_\D: \delta^u \overset{\wp}{\longleftrightarrow} \delta^t } \Prob{ e^{-1} \overset{\Lc_{\D \setminus \delta^t \D}^\theta}{\longleftrightarrow} \delta^u  } \d u
\end{align*}
We have obtained that
\begin{align*}
\Prob{e^{-1} \overset{\Lc_\D^\theta}{\longleftrightarrow} \delta^s}
= \Prob{e^{-1} \overset{\Lc_\D^\theta}{\longleftrightarrow} \delta^t }
+ \left( 1 - \Prob{ \exists \wp \in \Lc_\D: \delta^s \overset{\wp}{\longleftrightarrow} \delta^t } \right) \Prob{ e^{-1} \overset{\Lc_{\D \setminus \delta^t \D}^\theta}{\longleftrightarrow} \delta^s  } \\
- \int_s^t \frac{\d}{\d u} \Prob{ \exists \wp \in \Lc_\D: \delta^u \overset{\wp}{\longleftrightarrow} \delta^t } \Prob{ e^{-1} \overset{\Lc_{\D \setminus \delta^t \D}^\theta}{\longleftrightarrow} \delta^u  } \d u
\end{align*}

Also,
\begin{align*}
\Prob{e^{-1} \overset{\Lc_\D^\theta}{\longleftrightarrow} \delta^s}
= \left( 1 - \Prob{ \exists \wp \in \Lc_\D: \delta^s \overset{\wp}{\longleftrightarrow} \delta^t } \right) \Prob{ e^{-1} \overset{\Lc_{\D \setminus \delta^t \D}^\theta}{\longleftrightarrow} \delta^s  } \\
+ \int_0^s \frac{\d}{\d u} \Prob{ \exists \wp \in \Lc_\D^\theta: \delta^u \overset{\wp}{\longleftrightarrow} \delta^t } \Prob{ e^{-1} \overset{\Lc_{\D \setminus \delta^t \D}^\theta}{\longleftrightarrow} \delta^u  } \d u
\end{align*}
Which is basically the same equation.

\medskip

$s_1 < s_2 < t_0 < t_1 < t_2$.
\begin{align*}
\Prob{e^{-1} \overset{\Lc_{\D \setminus \delta^{t_2} \D}^\theta}{\longleftrightarrow} \delta^{s_1}}
= \left( 1 - \Prob{ \exists \wp \in \Lc_{\D \setminus \delta^{t_2} \D}: \delta^{s_1} \overset{\wp}{\longleftrightarrow} \delta^{t_1} } \right) \Prob{ e^{-1} \overset{\Lc_{\D \setminus \delta^{t_1} \D}^\theta}{\longleftrightarrow} \delta^{s_1}  } \\
+ \int_0^{s_1} \frac{\d}{\d u} \Prob{ \exists \wp \in \Lc_{\D \setminus \delta^{t_2} \D}^\theta: \delta^u \overset{\wp}{\longleftrightarrow} \delta^{t_1} } \Prob{ e^{-1} \overset{\Lc_{\D \setminus \delta^{t_1} \D}^\theta}{\longleftrightarrow} \delta^u  } \d u
\end{align*}
We now divide by $\Prob{e^{-1} \overset{\Lc_{\D \setminus \delta^{t_0} \D}^\theta}{\longleftrightarrow} \delta^{s_2}}$ and we define
\[
\phi_\delta(s_1,s_2,t_1,t_2) := \Prob{e^{-1} \overset{\Lc_{\D \setminus \delta^{t_2} \D}^\theta}{\longleftrightarrow} \delta^{s_1}} / \Prob{e^{-1} \overset{\Lc_{\D \setminus \delta^{t_1} \D}^\theta}{\longleftrightarrow} \delta^{s_2}}.
\]
\begin{align*}
\phi_\delta(s_1,s_2,t_0,t_2)
= \left( 1 - \Prob{ \exists \wp \in \Lc_{\D \setminus \delta^{t_2} \D}: \delta^{s_1} \overset{\wp}{\longleftrightarrow} \delta^{t_1} } \right) \phi_\delta(s_1,s_2,t_0,t_1) \\
+ \int_0^{s_1} \frac{\d}{\d u} \Prob{ \exists \wp \in \Lc_{\D \setminus \delta^{t_2} \D}^\theta: \delta^u \overset{\wp}{\longleftrightarrow} \delta^{t_1} } \phi_\delta(u,s_2,t_0,t_1) \d u
\end{align*}
\begin{align*}
\Prob{ \exists \wp \in \Lc_{\D \setminus \delta^{t_2} \D}: \delta^{s_1} \overset{\wp}{\longleftrightarrow} \delta^{t_1} }
= \Prob{ \exists \wp \in \Lc_\D: \delta^{s_1} \overset{\wp}{\longleftrightarrow} \delta^{t_1} } - \Prob{ \exists \wp \in \Lc_\D: \delta^{s_1} \overset{\wp}{\longleftrightarrow} \delta^{t_2} } \\
\to \left( \frac{t_2 - s_1}{t_2} \right)^\theta - \left( \frac{t_1 - s_1}{t_1} \right)^\theta
\end{align*}
and
\[
\frac{\d}{\d u} \Prob{ \exists \wp \in \Lc_{\D \setminus \delta^{t_2} \D}^\theta: \delta^u \overset{\wp}{\longleftrightarrow} \delta^{t_1} }
\to \theta \frac{(t_1-u)^{\theta-1}}{t_1^\theta} - \theta \frac{(t_2-u)^{\theta-1}}{t_2^\theta}
\]
\begin{align*}
\phi(s_1,s_2,t_0,t_2)
= \left( 1 - \left( \frac{t_2 - s_1}{t_2} \right)^\theta + \left( \frac{t_1 - s_1}{t_1} \right)^\theta \right) \phi(s_1,s_2,t_0,t_1) \\
+ \theta \int_0^{s_1} \left( \frac{(t_1-u)^{\theta-1}}{t_1^\theta} - \frac{(t_2-u)^{\theta-1}}{t_2^\theta} \right) \phi(u,s_2,t_0,t_1) \d u
\end{align*}

\bigskip

*******

Let $0 < s < t$ and $\delta >0$. 
\begin{align*}
\Prob{ e^{-1} \overset{\Lc_\D^\theta}{\longleftrightarrow} \delta^s }
= \Prob{ \nexists \wp \in \Lc_\D^\theta: \delta^s \overset{\wp}{\longleftrightarrow} \delta^t } \Prob{ e^{-1} \overset{\Lc_{\D \setminus \delta^t \D}^\theta}{\longleftrightarrow} \delta^s } \\
+ \int_0^s \frac{\d}{\d u} \Prob{ \exists \wp \in \Lc_\D^\theta: \delta^u \overset{\wp}{\longleftrightarrow} \delta^t } \Prob{ e^{-1} \overset{\Lc_{\D \setminus \delta^t \D}^\theta}{\longleftrightarrow} \delta^u } \d u
\end{align*}
Let us define
\[
\phi(s,t) = \lim_{\delta \to 0} \Prob{ e^{-1} \overset{\Lc_{\D \setminus \delta^t \D}^\theta}{\longleftrightarrow} \delta^s } / \Prob{ e^{-1} \overset{\Lc_{\D \setminus \delta^2 \D}^\theta}{\longleftrightarrow} \delta }
\]
and
\[
\psi(s) = \lim_{\delta \to 0} \Prob{ e^{-1} \overset{\Lc_{\D}^\theta}{\longleftrightarrow} \delta^s } / \Prob{ e^{-1} \overset{\Lc_{\D \setminus \delta^2 \D}^\theta}{\longleftrightarrow} \delta }.
\]
We have obtained that
\begin{align*}
\psi(s) = \left( \frac{t-s}{t} \right)^\theta \phi(s,t) + \theta \int_0^s \frac{(t-u)^{\theta-1}}{t^\theta} \phi(u,t) \d u.
\end{align*}
Since we believe that $\psi(s) = c_0 s^{-1+\theta}$, this equation allows us to find $\phi$. Indeed, defining $F(s,t) = \int_0^s \frac{(t-u)^{\theta-1}}{t^\theta} \phi(u,t) \d u$, the above equation can be rewritten as
\[
\frac{\partial F}{\partial s} = \frac{1}{t-s} \psi(s) - \frac{\theta}{t-s} F(s,t).
\]
\[
\frac{\partial}{\partial s} \left( (t-s)^{-\theta} F(s,t) \right) = (t-s)^{-\theta-1} \psi(s).
\]
Integrating,
\[
(t-s)^{-\theta} F(s,t) = \int_0^s (t-u)^{-\theta-1} \psi(u) \d u = \frac{c_0}{\theta} s^\theta (1-s/t)^{-\theta} t^{-1-\theta}.
\]
$F(s,t) = \frac{c_0}{\theta} s^\theta t^{-1}$. Differentiating w.r.t. $s$, we obtain that $\phi(s,t) = c_0 \left( \frac{t-s}{ts} \right)^{1-\theta}$. The constant $c_0$ can be identified by the fact that $\phi(1,2) = 1$.

\bigskip

$s < t_1 < t_2$.
\begin{align*}
\Prob{e^{-1} \overset{\Lc_{\D \setminus \delta^{t_2} \D}^\theta}{\longleftrightarrow} \delta^{s}}
= \Prob{ \nexists \wp \in \Lc_{\D \setminus \delta^{t_2} \D}: \delta^{s} \overset{\wp}{\longleftrightarrow} \delta^{t_1} } \Prob{ e^{-1} \overset{\Lc_{\D \setminus \delta^{t_1} \D}^\theta}{\longleftrightarrow} \delta^{s}  } \\
+ \int_0^{s} \frac{\d}{\d u} \Prob{ \exists \wp \in \Lc_{\D \setminus \delta^{t_2} \D}^\theta: \delta^u \overset{\wp}{\longleftrightarrow} \delta^{t_1} } \Prob{ e^{-1} \overset{\Lc_{\D \setminus \delta^{t_1} \D}^\theta}{\longleftrightarrow} \delta^u  } \d u
\end{align*}
Since
\begin{align*}
\Prob{ \nexists \wp \in \Lc_{\D}^\theta: \delta^{s} \overset{\wp}{\longleftrightarrow} \delta^{t_1} }
= \Prob{ \nexists \wp \in \Lc_{\D \setminus \delta^{t_2} \D}^\theta: \delta^{s} \overset{\wp}{\longleftrightarrow} \delta^{t_1} }
\Prob{ \nexists \wp \in \Lc_{\D}^\theta: \delta^{s} \overset{\wp}{\longleftrightarrow} \delta^{t_2} },
\end{align*}
\begin{align*}
\Prob{ \nexists \wp \in \Lc_{\D \setminus \delta^{t_2} \D}^\theta: \delta^{s} \overset{\wp}{\longleftrightarrow} \delta^{t_1} } \to \left( \frac{t_2}{t_1} \right)^\theta \left( \frac{t_1-s}{t_2-s} \right)^\theta
\end{align*}
and
\begin{align*}
\frac{\d}{\d u} \Prob{ \exists \wp \in \Lc_{\D \setminus \delta^{t_2} \D}^\theta: \delta^u \overset{\wp}{\longleftrightarrow} \delta^{t_1} }
\to \theta \left( \frac{t_2}{t_1} \right)^\theta (t_2-t_1) \frac{(t_1-u)^{\theta-1}}{(t_2-u)^{\theta+1}}.
\end{align*}
Overall we get the following equation for $\phi$:
\begin{align*}
\phi(s,t_2) = \left( \frac{t_2}{t_1} \right)^\theta \left( \frac{t_1-s}{t_2-s} \right)^\theta \phi(s,t_1) + \theta \left( \frac{t_2}{t_1} \right)^\theta (t_2-t_1) \int_0^s \frac{(t_1-u)^{\theta-1}}{(t_2-u)^{\theta+1}} \phi(u,t_1) \d u.
\end{align*}

==> subfiles/old_lower_bound_f.tex <==

\begin{lemma}\label{L:upper_bound_exponent}
The function $f_\infty$ satisfies
$
\int_1^\infty f_\infty(s) s^{-\theta} \d s = \infty.
$
\end{lemma}

\begin{proof}
Let $u : s \in (1,\infty) \mapsto (s-1)^{-\theta} (1-f_\infty(s)) \in [0,\infty)$.
The fact that $Tf_\infty = f_\infty$ implies that for all $t > 1$,
\begin{equation}
\label{E:proof_infinity}
u(t) = \theta \int_1^\infty (s-1)^\theta (s+t-1)^{-\theta -1} u(s) \d s.
\end{equation}
This in particular implies that $u(s)$ has a finite limit as $s \to 1^+$.
We now compute the integral of $u$ times $f_\infty$. All the terms involved below are nonnegative, so we can safely exchange integrals and we obtain by definition of $T_\infty$:
\begin{align*}
& \int_1^\infty u(s) f_\infty(s) \d s
= \int_1^\infty u(s) T f_\infty (s) \d s \\
& = \int_1^\infty u(s) \Big( 1 - \Big(1-\frac1{s}\Big)^\theta \Big) \d s
+ \int_1^\infty f_\infty(t) \left( \theta \int_1^\infty (s-1)^\theta (s+t-1)^{-\theta-1} u(s) \d s \right) \d t.
\end{align*}
Using \eqref{E:proof_infinity} we deduce that
\begin{align*}
& \int_1^\infty u(s) f_\infty(s) \d s
= \int_1^\infty u(s) \Big( 1 - \Big(1-\frac1{s}\Big)^\theta \Big) \d s
+ \int_1^\infty u(t) f_\infty(t) \d t.
\end{align*}
The first integral on the right hand side being positive, the integral of $u$ times $f_\infty$ has to be infinite. This concludes the proof since $u(s)$ has a finite limit as $s \to 1^+$ and $u(s) \sim s^{-\theta}$ as $s \to \infty$.
\end{proof}

